Point Cloud Instance Segmentation using Probabilistic Embeddings

In this paper we propose a new framework for point cloud instance segmentation. Our framework has two steps: an embedding step and a clustering step. In the embedding step, our main contribution is to propose a probabilistic embedding space for point cloud embedding. Specifically, each point is represented as a tri-variate normal distribution. In the clustering step, we propose a novel loss function, which benefits both the semantic segmentation and the clustering. Our experimental results show important improvements to the SOTA, i.e., 3.1% increased average per-category mAP on the PartNet dataset.

==> data_tex/ap-iou.tex <==
%auto-ignore
\begin{table}
\caption{\textbf{Results on PartNet} (Overall average part-category mAP\%, different IoU thresholds).}
\centering
\begin{tabular}{@{}llll@{}}
\toprule
% & \multicolumn{3}{c}{IoU threshold} \\
IoU threshold & 0.25 & 0.50 & 0.75 \\ \midrule
PartNet & 62.8 & 54.4 & 38.9 \\
Ours & \textbf{66.5} & \textbf{57.5} & \textbf{41.7} \\ \bottomrule
\end{tabular}
\label{tbl:iou}
\end{table}

==> data_tex/part-stat.tex <==
%auto-ignore
\begin{table*}[]
\small\addtolength{\tabcolsep}{-4.7pt}
\caption{\textbf{PartNet statistics}. We show number of samples, num of classes and number of instances per sample here (coarse(1)-, middle(2)-, and fine-grained(3)). We also hightlight four largest categories.}
\label{tbl:part-stat}
\centering
\resizebox{\columnwidth}{!}{%
% \small\addtolength{\tabcolsep}{-5.5pt}
% \begin{tabular}{llllllllllllllllllllllllll}
% \begin{tabular}{@{}clrrrrrrrrrrrrrrrrrrrrrrrr@{}}
\begin{tabular}{@{}clcccccccccccccccccccccccc@{}}
\toprule
 &     & \rotatebox[origin=lB]{90}{Bag}  & \rotatebox[origin=lB]{90}{Bed}  & \rotatebox[origin=lB]{90}{Bottle} & \rotatebox[origin=lB]{90}{Bowl} & \rotatebox[origin=lB]{90}{Chair} & \rotatebox[origin=lB]{90}{Clock} & \rotatebox[origin=lB]{90}{Dish} & \rotatebox[origin=lB]{90}{Disp} & \rotatebox[origin=lB]{90}{Door} & \rotatebox[origin=lB]{90}{Ear}  & \rotatebox[origin=lB]{90}{Faucet} & \rotatebox[origin=lB]{90}{Hat}  & \rotatebox[origin=lB]{90}{Key}  & \rotatebox[origin=lB]{90}{Knife} & \rotatebox[origin=lB]{90}{Lamp} & \rotatebox[origin=lB]{90}{Laptop}   & \rotatebox[origin=lB]{90}{Micro} & \rotatebox[origin=lB]{90}{Mug}  & \rotatebox[origin=lB]{90}{Fridge} & \rotatebox[origin=lB]{90}{Scis} & \rotatebox[origin=lB]{90}{Stora} & \rotatebox[origin=lB]{90}{Table} & \rotatebox[origin=lB]{90}{Trash} & \rotatebox[origin=lB]{90}{Vase} \\ \midrule
 \multirow{3}{*}{samples} & train & 92   & 133   & 315    & 131  & \textbf{4489}  & 406   & 111        & 633     & 149  & 147      & 435    & 170  & 111      & 221   & \textbf{1554} & 306    & 133       & 138  & 136          & 45       & \textbf{1588}             & \textbf{5707}  & 221      & 741  \\
 & val & 5    & 24    & 37     & 18   & \textbf{617}   & 50    & 19         & 104     & 25   & 28       & 81     & 16   & 14       & 29    & \textbf{234}  & 45     & 12        & 19   & 20           & 10       & \textbf{230}              & \textbf{843}   & 37       & 102  \\
 & test & 29   & 37    & 84     & 39   & \textbf{1217}  & 98    & 51         & 191     & 51   & 53       & 132    & 45   & 31       & 77    & \textbf{419}  & 82     & 39        & 35   & 31           & 13       & \textbf{451}              & \textbf{1668}  & 63       & 233  \\ \midrule
\multirow{3}{*}{classes} & 1 & 3    & 3     & 5      & 3    & \textbf{5}     & 5     & 2          & 2       & 2    & 5        & 7      & 5    & 2        & 4     & \textbf{17}   & 2      & 2         & 3    & 2            & 2        & \textbf{6}                & \textbf{10}    & 4        & 3    \\
 & 2 & -    & 9     & -      & -    & \textbf{29}    & -     & 4          & -       & 3    & -        & -      & -    & -        & -     & \textbf{27}   & -      & 4         & -    & 5            & -        & \textbf{18}               & \textbf{41}    & -        & -    \\
 & 3 & -    & 14    & 8      & -    & \textbf{38}    & 10    & 6          & 3       & 4    & 9        & 11     & -    & -        & 9     & \textbf{40}   & -      & 5         & -    & 6            & -        & \textbf{23}               & \textbf{50}    & 10       & 5    \\ \midrule
\multirow{3}{1.5cm}{instances per sample} & 1 & 3.08 & 3.56  & 2.63   & 1.52 & \textbf{3.92}  & 1.88  & 1.74       & 1.86    & 1.53 & 3.23     & 3.94   & 2.64 & 99.52    & 2.02  & \textbf{2.74} & 2.54   & 1.23      & 2.46 & 1.47         & 4.78     & \textbf{7.02}             & \textbf{2.07}  & 2.81     & 1.51 \\
 & 2 & -    & 15.19 & -      & -    & \textbf{10.13} & -     & 3.47       & -       & 2.65 & -        & -      & -    & -        & -     & \textbf{4.17} & -      & 3.45      & -    & 3.88         & -        & \textbf{19.00}            & \textbf{9.65}  & -        & -    \\
 & 3 & -    & 30.71 & 2.83   & -    & \textbf{12.97} & 3.85  & 5.14       & 2.67    & 3.75 & 6.69     & 6.50   & -    & -        & 3.37  & \textbf{5.56} & -      & 4.51      & -    & 6.62         & -        & \textbf{21.54}            & \textbf{11.20} & 20.21    & 2.12 \\ \bottomrule
\end{tabular}
}
\end{table*}

==> fig_tex/sim-measure.tex <==
%auto-ignore
\tikzfading
[
  name=fade out,
  inner color=transparent!0,
  outer color=transparent!100
]
\tikzset{rv/.style={red,path fading=fade out,}}
\begin{figure}[tb]
    \centering
    \begin{subfigure}{0.25\linewidth}
        % \includegraphics[width=\textwidth]{example-image-a}
        \begin{tikzpicture}
            \begin{axis}[
                scale only axis,
                width=0.8\textwidth,
                height=0.8\textwidth,
                xmin=0,xmax=3,
                ymin=0,ymax=3,
                xticklabel=\empty,
                yticklabel=\empty,
                axis lines = middle
            ]
            \addplot[color = black, mark=*] coordinates {
            (1, 2)
            (2, 1)
            } node[above, pos=0]{$\mathbf{e}_i$} node[below, pos=1.0]{$\mathbf{e}_j$};
            \end{axis}
        \end{tikzpicture}
        \caption{Euclidean}
        % \label{fig:my_label}
    \end{subfigure}%
    \begin{subfigure}{0.25\linewidth}
        % \includegraphics[width=\textwidth]{example-image-a}
        \begin{tikzpicture}
            \begin{axis}[
                scale only axis,
                width=0.8\textwidth,
                height=0.8\textwidth,
                xmin=0,xmax=3,
                ymin=0,ymax=3,
                xticklabel=\empty,
                yticklabel=\empty,
                axis lines = middle
            ]
            \addplot[color = black, mark=*] coordinates {
            (0, 0)
            (1, 2)
            } node[above, pos=1]{$\mathbf{e}_i$};
            \addplot[color = black, mark=*] coordinates {
            (0, 0)
            (2, 1)
            } node[below, pos=1]{$\mathbf{e}_j$};
            \path 
                (1, 0.5)node[](A){} 
                (0.5, 1)node[](B){}
                (0, 0)node[](O){};
            \end{axis}
            \tkzMarkAngle[](A,O,B);
        \end{tikzpicture}
        \caption{Cosine}
        % \label{fig:my_label}
    \end{subfigure}%
    \begin{subfigure}{0.25\linewidth}
        \begin{tikzpicture}
            \begin{axis}[
                scale only axis,
                width=0.8\textwidth,
                height=0.8\textwidth,
                xmin=0,xmax=3,
                ymin=0,ymax=3,
                xticklabel=\empty,
                yticklabel=\empty,
                axis lines = middle
            ]
                \addplot[color = black, mark=*] coordinates {
                    (1, 2)
                } node[above, pos=1]{$\mathbf{e}_i$};
                \fill[rv] (1,2) ellipse [x radius=1, y radius=0.5];
                \addplot[color = black, mark=*] coordinates {
                    (2, 1)
                } node[below, pos=1]{$\mathbf{e}_j$};
                \fill[rv,color = blue] (2,1) ellipse [x radius=0.7, y radius=1.0];
            \end{axis}
        \end{tikzpicture}
        \caption{Probabilistic}
    \end{subfigure}%
    \caption{Examples of (dis)similarity measures}
    \label{fig:euc-cos}
\end{figure}
